Mapping Navigation Instructions to Continuous Control Actions with Position-Visitation Prediction

We propose an approach for mapping natural language instructions and raw observations to continuous control of a quadcopter drone. Our model predicts interpretable position-visitation distributions indicating where the agent should go during execution and where it should stop, and uses the predicted distributions to select the actions to execute. This two-step model decomposition allows for simple and efficient training using a combination of supervised learning and imitation learning. We evaluate our approach with a realistic drone simulator, and demonstrate absolute task-completion accuracy improvements of 16.85% over two state-of-the-art instruction-following methods.

==> sup.tex <==
\input{header} 

%
%
%
%
\title{Mapping Navigation Instructions to Continuous Control Actions with Position-Visitation Prediction \\ (Supplementary Material)}

\begin{document}
\maketitle

\input{appendix}

%
%
%
%


\end{document}

